PeLiCal: Targetless Extrinsic Calibration via Penetrating Lines for RGB-D Cameras with Limited Co-visibility

RGB-D cameras are crucial in robotic perception, given their ability to produce images augmented with depth data. However, their limited FOV often requires multiple cameras to cover a broader area. In multi-camera RGB-D setups, the goal is typically to reduce camera overlap, optimizing spatial coverage with as few cameras as possible. The extrinsic calibration of these systems introduces additional complexities. Existing methods for extrinsic calibration either necessitate specific tools or highly depend on the accuracy of camera motion estimation. To address these issues, we present PeLiCal, a novel line-based calibration approach for RGB-D camera systems exhibiting limited overlap. Our method leverages long line features from surroundings, and filters out outliers with a novel convergence voting algorithm, achieving targetless, real-time, and outlier-robust performance compared to existing methods. We open source our implementation on https://github.com/joomeok/PeLiCal.git.

==> note.tex <==
# Free Notes


% %FIGURE
% \begin{figure}[!t]
%     \centering
%    % \vspace{-1mm}
%     \subfloat[Overlap of two images\label{fig:feature_overlap1}]{
% 		\includegraphics[height=0.48\columnwidth]{./figs/overlap.png}
%     }
%     \subfloat[Revloution scan delay\label{fig:feature_overlap2}]{
% 		\includegraphics[height=0.48\columnwidth]{./figs/overlap2.png}
% 	}\\
%     \subfloat[Contour and nearest point extraction\label{fig:feature_contour}]{
% 		\includegraphics[width=0.98\columnwidth]{./figs/features.pdf}
% 	}
%     \vspace{-1mm}
%     \caption{(a) In our dataset, certain regions remain un-updated due to the low update rate. An accumulation in these overlapping areas could lead to unexpected convergence behaviors. (b) Given that radar imagery inherently constitutes scan-rotated images, there exists a discrepancy between the commencement and conclusion of the scans, primarily attributed to temporal lags. This discrepancy is especially pronounced during sharp rotational movements. (c) Initially, we delineate the contour, subsequently identifying proximal points to ensure consideration extends beyond just the central points.}
%     \label{fig:feature}
%     \vspace{-5mm}
% \end{figure}


% %FIGURE
% \begin{figure}[!t]
%     \centering
%    % \vspace{-1mm}
%     \includegraphics[width=0.98\columnwidth]{./figs/fig3.pdf}
%     \vspace{-1mm}
%     \caption{Concept of the LodeStar Descriptor. From the primary radar imagery, we compute a radial intensity vector for every $\theta$. Each of these vectors is subsequently integrated to constitute a column within the integrated radial intensity matrix. By iterating this process over a period of 2$\pi$, we synthesize the final descriptor.}
%     \label{fig:lodestar}
%     \vspace{-5mm}
% \end{figure}


root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-48-03_minmax/recall_rates.csv 
STHEREO-SNU, 56.73, 74.61, 80.08, 84.90
STHEREO-valley, 83.60, 96.46, 98.71, 99.36
vivid-urban, 92.22, 98.13, 99.22, 99.69
vivid-city, 92.02, 96.55, 98.17, 98.99

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-49-24_histeq/recall_rates.csv 
STHEREO-SNU, 63.02, 79.35, 84.41, 88.33
STHEREO-valley, 75.88, 89.39, 94.53, 96.14
vivid-urban, 91.91, 98.29, 98.91, 99.69
vivid-city, 89.25, 97.84, 98.78, 99.19

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-50-31_minmax_gridwise_8x8/recall_rates.csv 
STHEREO-SNU, 53.55, 75.02, 81.31, 86.69
STHEREO-valley, 50.80, 71.38, 76.85, 81.99
vivid-urban, 88.49, 96.58, 98.76, 99.53
vivid-city, 91.62, 96.08, 97.50, 98.65

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-51-45_minmax_gridwise_message_passing_8x8_mean_3/recall_rates.csv 
STHEREO-SNU, 61.80, 79.51, 85.22, 89.80
STHEREO-valley, 87.78, 97.43, 98.71, 99.04
vivid-urban, 93.78, 98.44, 99.07, 99.84
vivid-city, 92.97, 96.08, 97.57, 98.51

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-53-10_minmax_gridwise_message_passing_8x8_mean_5/recall_rates.csv 
STHEREO-SNU, 60.33, 77.80, 81.80, 87.27
STHEREO-valley, 90.03, 96.78, 98.07, 99.36
vivid-urban, 94.40, 99.22, 99.38, 99.84
vivid-city, 91.35, 96.42, 97.70, 98.65

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-54-42_minmax_gridwise_message_passing_16x16_mean_3/recall_rates.csv 
STHEREO-SNU, 65.71, 80.24, 84.33, 89.06
STHEREO-valley, 76.21, 91.00, 95.18, 96.78
vivid-urban, 92.07, 97.51, 99.07, 100.00
vivid-city, 90.40, 96.35, 97.77, 98.65

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-55-56_minmax_gridwise_message_passing_16x16_mean_5/recall_rates.csv 
STHEREO-SNU, 59.67, 77.55, 83.51, 88.24
STHEREO-valley, 76.85, 90.03, 95.50, 97.43
vivid-urban, 89.27, 97.20, 99.07, 99.84
vivid-city, 90.94, 95.47, 97.63, 98.58

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-57-11_minmax_gridwise_message_passing_16x16_mean_7/recall_rates.csv 
STHEREO-SNU, 60.90, 78.94, 84.90, 88.82
STHEREO-valley, 78.46, 93.89, 97.43, 99.36
vivid-urban, 90.82, 97.67, 99.38, 99.84
vivid-city, 90.80, 96.15, 97.90, 98.99

